Backpropagation and Biological Plausibility

By and large, Backpropagation (BP) is regarded as one of the most important neural computation algorithms at the basis of the progress in machine learning, including the recent advances in deep learning. However, its computational structure has been the source of many debates on its arguable biological plausibility. In this paper, it is shown that when framing supervised learning in the Lagrangian framework, while one can see a natural emergence of Backpropagation, biologically plausible local algorithms can also be devised that are based on the search for saddle points in the learning adjoint space composed of weights, neural outputs, and Lagrangian multipliers. This might open the doors to a truly novel class of learning algorithms where, because of the introduction of the notion of support neurons, the optimization scheme also plays a fundamental role in the construction of the architecture.

==> ContinuumSetting.tex <==
Suppose we are dealing with learning tasks with an inherent temporal structure.
In this case, one formulate learning in the framework of the least cognitive action principle.
We define the cognitive action as
\begin{equation}
	A(w) = \int_{0}^{T} \bigg( \frac{1}{2} m_{i} \dot{w}_{i}^{2}   - V(w,x) \bigg)dt
\end{equation}

==> OnLine.tex <==
The extension of the 

==> mydefs.tex <==

% For et al.'ing things
\newcommand{\etal}{{\em et al.\/}}
\def\annote#1{\par {\bf #1}\par}

\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbN}{{\mathbb{N}}}

%\def\NaturalSet{\mbox{I\hspace*{-0.16em}N}}
\def\RealSet{\mbox{I\hspace*{-0.16em}R}}

\def\NaturalSet{\mbox{$I\!\! N$}}
%\def\RealSet{\mbox{$I\!\!R$}}
%\def\func#1{\mbox{$#1(\cdot)$}}

\def\N{\mbox{$I\!\! N$}}
\def\R{\mbox{$I\!\!R$}}
\def\C{\mbox{\rm C}}

\def\QED{\protect{\flushright{$\Box$}}}
%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\def\qed{\hspace*{\fill}~\protect{\QED}}
%\def\ONE{\Huge{\bf 1}\hspace{-.1cm}\normalsize{\mbox {\bf I}}}
\def\ONE{{\bf 1}\hspace{-.1cm}{\mbox {\bf I}}}
\def\ZERO{\bf 0}

\def\sequence#1#2#3{#1^{#3\choose #2}}
\def\chain{\oplus}
\def\quantize#1{\ulcorner #1 \lrcorner}
\def\path{\leadsto}
\def\nil{\mbox{\boldmath $0$}} 
\def\ONE{\mbox{\boldmath $1$}} 
\def\BBox{\vrule height 1.2ex width 1.2ex depth -.1ex}
\def\warp{\bowtie}
\def\RealSet{\mbox{$I\!\!R$}}
\def\Kernel{\mbox{$I\!\!K$}}

\def\smap{F}
\def\gmap{\mbox{\Large{$\tau$}}}
\def\tmap{f}


\def\shape#1{\rm }
\def\ot{\overline{t}}
\def\osigma{\overline{\sigma}}
\def\Set{\mbox{$\mbox{\sc set}$}}
\def\Reset{\mbox{$\mbox{\sc reset}$}}
\def\Nil{\mbox{$\mbox{\sc nil}$}}
\def\Not{\mbox{$\mbox{\sc not}$}}
\def\False{\mbox{$\mbox{\sc false}$}}
\def\True{\mbox{$\mbox{\sc true}$}}

\def\Action{$\mbox{\boldmath ${\cal A}$}$}

\def\pa{\mbox{pa}}
\def\vert{\mbox{vert}}
\def\de{\mbox{de}}
\def\det{\mbox{det}}
\def\dim{\mbox{dim}}
\def\sign{\mbox{sign}}
\def\diag{\mbox{diag}}
\def\ln{\mbox{ln}}
%\def\arg{\mbox{\shape{n}\selectfont arg}}
\def\softmax{\mbox{softmax}}
\def\argmax{\mathop{\operator@font argmax}}
\def\argmin{\mathop{\operator@font argmin}}

\def\BA{\mbox{\boldmath $A$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BD{\mbox{\boldmath $D$}}
\def\BG{\mbox{\boldmath $G$}}
\def\BF{\mbox{\boldmath $F$}}
\def\BI{\mbox{\boldmath $I$}} 
\def\BPhi{\mbox{\boldmath $\Phi$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BS{\mbox{\boldmath $S$}} 
\def\BL{\mbox{\boldmath $L$}} 
\def\BTheta{\mbox{\boldmath $\Theta$}}
\def\BU{\mbox{\boldmath $U$}} 
\def\BH{\mbox{\boldmath $H$}} 
\def\BM{\mbox{\boldmath $M$}}
\def\BN{\mbox{\boldmath $N$}}
\def\BP{\mbox{\boldmath $P$}} 
\def\BT{\mbox{\boldmath $T$}}
\def\BV{\mbox{\boldmath $V$}} 
\def\BX{\mbox{\boldmath $X$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BY{\mbox{\boldmath $Y$}} 
\def\BW{\mbox{\boldmath $W$}}
\def\BZ{\mbox{\boldmath $Z$}}
\def\B0{\mbox{\boldmath $0$}}
\def\Balpha{\mbox{\boldmath $\alpha$}}
\def\Ba{\mbox{\boldmath $a$}}
\def\Bbeta{\mbox{\boldmath $\beta$}}
\def\Bb{\mbox{\boldmath $b$}}
\def\Bc{\mbox{\boldmath $c$}}
\def\Bd{\mbox{\boldmath $b$}}
\def\Bgamma{\mbox{\boldmath $\gamma$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\BDelta{\mbox{\boldmath $\Delta$}}
\def\Beta{\mbox{\boldmath $\eta$}}
\def\Be{\mbox{\boldmath $e$}}
\def\Bepsilon{\mbox{\boldmath $\epsilon$}}
\def\Bf{\mbox{\boldmath $f$}}
\def\Bn{\mbox{\boldmath $n$}}
\def\Blambda{\mbox{\boldmath $\lambda$}}
\def\Bg{\mbox{\boldmath $g$}}
\def\Bmu{\mbox{\boldmath $\mu$}} 
\def\Bnu{\mbox{\boldmath $\nu$}} 
\def\Bm{\mbox{\boldmath $m$}}
\def\Bo{\mbox{\boldmath $o$}}
\def\Bphi{\mbox{\boldmath $\phi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bpsi{\mbox{\boldmath $\psi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bp{\mbox{\boldmath $p$}}
\def\Bq{\mbox{\boldmath $q$}}
\def\Br{\mbox{\boldmath $r$}}
\def\Bs{\mbox{\boldmath $s$}}
\def\B\tau{\mbox{\boldmath $\tau$}}
\def\Btheta{\mbox{\boldmath $\theta$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\Bomega{\mbox{\boldmath $\omega$}}
\def\Bu{\mbox{\boldmath $u$}}
\def\Bvarphi{\mbox{\boldmath $\varphi$}}
\def\Bvartheta{\mbox{\boldmath $\vartheta$}}
\def\Bvarsigma{\mbox{\boldmath $\varsigma$}}
\def\Bv{\mbox{\boldmath $v$}}
\def\Bw{\mbox{\boldmath $w$}} 
\def\Bxi{\mbox{\boldmath $\xi$}}
\def\Bx{\mbox{\boldmath $x$}}
\def\Bd{\mbox{\boldmath $d$}}
\def\By{\mbox{\boldmath $y$}} 
\def\Bzeta{\mbox{\boldmath $\zeta$}}
\def\Bz{\mbox{\boldmath $z$}}
\def\EQ{\!=\!}
\def\Given{\mbox{$\: \bigl | \bigr. \:$}}
\def\MAX{\mbox{\sc max}}
\def\MIN{\mbox{\sc min}}
\def\Overq{{\overline{q}}}
\def\Pr{\mbox{P}}
\def\given{\mbox{$\: | \:$}}

\def\vectw#1#2{\!\left[\!\!\begin{array}{r}#1\\#2\end{array}\!\!\right]\!}

\def\ivector#1{\sfmath{I}_{[#1]}}
\def\CalA{{\cal A}}
\def\CalB{{\cal B}}
\def\CalC{{\cal C}}
\def\CalD{{\cal D}}
\def\CalE{{\cal E}}
\def\CalF{{\cal F}}
\def\CalG{{\cal G}}
\def\CalH{{\cal H}}
\def\CalI{{\cal I}}
\def\CalJ{{\cal J}}
\def\CalL{{\cal L}}
\def\CalM{{\cal M}}
\def\CalN{{\cal N}}
\def\CalO{{\cal O}}
\def\CalP{{\cal P}}
\def\CalQ{{\cal Q}}
\def\CalR{{\cal R}}
\def\CalS{{\cal S}}
\def\CalT{{\cal T}}
\def\CalU{{\cal U}}
\def\CalV{{\cal V}}
\def\CalW{{\cal W}}
\def\CalX{{\cal X}}
\def\CalY{{\cal Y}}
\def\CalZ{{\cal Z}}
\def\VecCalE{{\cal{\vec{E}}}}
\def\Alphabet{{\cal A}}
\def\Real{\mbox{$\mathbb{R}$}}
\def\AND{\mbox{${\cal B}_\wedge$}}
\def\OR{\mbox{${\cal B}_\vee$}}

\def\istar{\mbox{$\CalI^\star$}}
% \def\EqDef{\doteq}
\def\EqDef{\buildrel \rm def \over =}

\def\RefFig#1{Figure~\ref{#1}}
\def\RefTab#1{Table~\ref{#1}}
\def\RefEq#1{(\ref{#1})}
\def\RefEqs#1#2{(\ref{#1},\ref{#2})}
\def\RefCh#1{Chapter \ref{#1}}
\def\RefSect#1{\S~\ref{#1}}
\def\RefSec#1{\S~\ref{#1}}
\def\RefSub#1{\S~\ref{#1}}
\def\RefDef#1{Definition~\ref{#1}}
\def\RefTh#1{Theorem~\ref{#1}}
\def\RefTh#1{Conjecture~\ref{#1}}
\def\cdw#1{{\em \underline{#1}}}


% An list-like environment that indents second, etc. lines of each item.
\newenvironment{defs}%
{\begin{list}{}{\setlength{\itemindent}{-\leftmargin}\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}}}%
{\end{list}}

% shrink and rotate everything for a two-pages on 1 printing using dvips.
%\input reduce.tex

% ``\heading'' is like a subsubsubsection, and takes a single argument.
% \newcommand{\heading}[1]{ \medskip
%         {\setlength{\parindent}{0in} \bf #1}
%         \nopagebreak
%         }

% ``\comment'' takes a single argument
\newcommand{\comment}[1]{}


% Local Variables: 
% mode: latex
% TeX-master: "main"
% End: 

